Constraining primordial non-Gaussianity from DESI quasar targets and Planck CMB lensing

We detect the cross-correlation between 2.7 million DESI quasar targets across 14,700 deg$^2$ (180 quasars deg$^{-2}$) and Planck 2018 CMB lensing at $\sim$30$\sigma$. We use the cross-correlation on very large scales to constrain local primordial non-Gaussianity via the scale dependence of quasar bias. The DESI quasar targets lie at an effective redshift of 1.51 and are separated into four imaging regions of varying depth and image quality. We select quasar targets from Legacy Survey DR9 imaging, apply additional flux and photometric redshift cuts to improve the purity and reduce the fraction of unclassified redshifts, and use early DESI spectroscopy of 194,000 quasar targets to determine their redshift distribution and stellar contamination fraction (2.6%). Due to significant excess large-scale power in the quasar autocorrelation, we apply weights to mitigate contamination from imaging systematics such as depth, extinction, and stellar density. We use realistic contaminated mocks to determine the greatest number of systematic modes that we can fit, before we are biased by overfitting and spuriously remove real power. We find that linear regression with one to seven imaging templates removed per region accurately recovers the input cross-power, $f_{\textrm{NL}}$ and linear bias. As in previous analyses, our $f_{\textrm{NL}}$ constraint depends on the linear primordial non-Gaussianity bias parameter, $b_{\phi} = 2(b - p)\delta_c$ assuming universality of the halo mass function. We measure $f_{\textrm{NL}} = -26^{+45}_{-40}$ with $p=1.6$ $(f_{\textrm{NL}} = -18^{+29}_{-27}$ with $p=1.0$), and find that this result is robust under several systematics tests. Future spectroscopic quasar cross-correlations with Planck lensing lensing can tighten the $f_{\textrm{NL}}$ constraints by a factor of 2 if they can remove the excess power on large scales in the quasar auto power spectrum.

==> notes.tex <==
\begin{document}

\section{Agenda}

1. Demonstrate that we can recover unbiased constraints
from fnl=0 mocks. Test on nonzero fnl mocks as well (Gaussian is fine).  Can also compare to Fisher forecasts.

1a. Need to include magnification in the mocks that I already have. (Need to measure magnification on the data sample by perturbing photometry
and re-running target selection).

1b.  Need to have some argument (at least) about linear/nonlinear power, if not
a full comparison to mocks.

1c. Show transfer function test.

1d. Discussion on covariance matrix.  Estimate the additional ``realization bias'' factor from mocks. Compare to Gaussian covariance matrix.

2. Impacts of redshift uncertainty.

3. Run on data.

\section{Notes}

Some additional issues that need to be addressed:

Add bias uncertainty to fnl constraints.

Uncertainty in theory: lmax, nonlinear modelling.

Uncertainty in covariance (corrections in Ho et al).

Magnification bias

Impact of uncertainty in redshift distribution. Is the mean the moment that matters, or the second moment (or something else) more relevant?

Other relativistic terms

Impact of varying redshift distribution on clustering. Can study this using mocks. Does it matter that the redshift distribution isn't constant on the sky?


I finally found what I was looking for when we spoke yesterday. I’d thought it was related to one of the papers where I had previously used Gaussian mocks with f_nl included in P(k), but it was actually related to a paper where we used a posterior shape derived for a Gaussian, but instead used this posterior to constrain f_nl. It’s the same problem - f_nl in the power is a first order correction compared to the other non-Gaussian effects. The relevant paper is:

https://arxiv.org/pdf/1504.03979.pdf

and the paragraph:

Here we work to first order in $\delta$,
so that we can continue to assume that $\delta_k$ is drawn from a Gaussian
distribution, with an altered $P(k)$, i.e. the first order effect of non-Gaussianity
is to $P_H(k)$, keeping the distribution the same. Furthermore, we do
not alter $V_n$ (Eq.\ (24)) to include any coupling between modes from the non-Gaussian signal.
Where $k$ is very small, higher order corrections to $\delta$ will become increasingly
important (e.g.\ Tellarini et al.\ 2015), suggesting that the Gaussian limit for $\delta$
will break down here.

\end{document}
